Long-Range Correlations of Sequences Modulo 1

In this paper we consider the fractional parts of a general sequence, for example the sequence $\alpha \sqrt{n}$ or $\alpha n^2$. We give a general method, which allows one to show that long-range correlations (correlations where the support of the test function grows as we consider more points) are Poissonian. We show that these statements about convergence can be reduced to bounds on associated Weyl sums. In particular we apply this methodology to the aforementioned examples. In so doing, we recover a recent result of Technau-Walker (2020) for the triple correlation of $\alpha n^2$ and generalize the result to higher moments. For both of the aforementioned sequences this is one of the only results which indicates the pseudo-random nature of the higher level ($m \ge 3$) correlations.

==> Chapters/OLD/4_Stationary_Phase_Integrals.tex <==


\section{The Remainder Term -- $m=2$}
\label{s:The Remainder Term 2}

It remains to estimate the remainder:

\begin{align*}
  \cE := \frac{1}{N} \sum_{0 \neq \vect{r}\hspace{-1mm} \Mod{q}} \left(\prod_{i=1}^m F_N(r_i)\right) \sum_{\vect{a} \in sI}^\ast \wh{h}_{\vect{a}}(\vect{r}).
\end{align*}

\textbf{First fix $m=2$} and rewrite the error term:

\begin{align*}
  \cE= \frac{1}{Nq^2} \sum_{\vect{x} \in \{1,\dots,q\}^2}^* \sum_{m \in \Z}\sum_{0 \neq \vect{r} \Mod{q}} \mathbbm{1}_{\frac{1}{N}I}(\beta(\vect{x}) + m )  e \left(-\frac{\vect{r}\cdot \vect{x}}{q}\right) \left( \prod_{i=1}^m F_N(r_i)\right),
\end{align*}
where $\beta(\vect{x}) : = \frac{b}{q}(\sqrt{x_1}-\sqrt{x_2})$ and the $\ast$ implies $x_1\neq x_2$.

To bound $\cE$, we first want to ignore the fact that $x_1$ and $x_2$ are distinct, thus write $\cE$ as the difference:

\begin{align*}
  \cE &= \frac{1}{Nq^2} \sum_{\vect{x} \in \{1,\dots,q\}^2} \sum_{m \in \Z}\sum_{0 \neq \vect{r} \Mod{q}} \mathbbm{1}_{\frac{1}{N}I}(\beta(\vect{x}) + m )  e \left(-\frac{\vect{r}\cdot \vect{x}}{q}\right) \left( \prod_{i=1}^m F_N(r_i)\right)\\
  & \phantom{++++} - \frac{1}{Nq^2} \sum_{x_1 \in \{1,\dots,q\}} \sum_{m \in \Z}\sum_{0 \neq \vect{r} \Mod{q}} \mathbbm{1}_{\frac{1}{N}I}( m )  e \left(-\frac{(r_1+r_2)x_1}{q}\right) \left( \prod_{i=1}^m F_N(r_i)\right)
\end{align*}
Now if $0 \not\in I$ then the second term is $0$ (for $N$ large enough). However if $0 \in I$ then the second term can be written


\begin{align*}
   \frac{1}{Nq^2} \sum_{0 \neq \vect{r} \Mod{q}}\left( \prod_{i=1}^m F_N(r_i)\right)  \left( \sum_{x_1 \in \{1,\dots,q\}}  e \left(-\frac{(r_1+r_2)x_1}{q}\right)\right) 
\end{align*}
this sum is $0$ unless $r_1+r_2 = q$. Thus, using \eqref{F bound}


\begin{align*}
   = \frac{1}{Nq} \sum_{\substack{0 \neq \vect{r} \Mod{q}\\ r_1+r_2=q} }\left( \prod_{i=1}^m F_N(r_i)\right) \ll \frac{1}{Nq} \sum_{\substack{0 \neq \vect{r} \Mod{q}\\ r_1+r_2=q} } \frac{q^2}{\abs{r_1r_2}}
\end{align*}
Now if $r_1+r_2 = q$ then we know either $r_1$ or $r_2 > \frac{q}{2}$ and we can estimate the sum by 

\begin{align*}
 \frac{1}{Nq} \sum_{r_1+r_2=q}  \frac{q^2}{\abs{r_1r_2}} \le \frac{2}{Nq} \sum_{r_2=1}^q  \frac{2q}{\abs{r_2}}  = \cO\left( \frac{1}{N}  \log q\right) \to 0
\end{align*}



%First we separate the sum over $r_1$ into three terms: one with $r_1=0$, one with $r_2=0$ and one with $r_1,r_2>0$. By symmetry we thus need to bound: 


% \begin{align*}
%   \cE_0 &= \frac{1}{q^2} \sum_{\vect{x} \in \{1,\dots,q\}^2} \sum_{m \in \Z}\hspace{2mm}\sum_{r_2 \in \{1,\dots,q-1\}} \mathbbm{1}_{\frac{1}{N}I}(\beta(\vect{x}) + m )  e \left(-\frac{r_2 x_2}{q}\right) F_{N}(r_2),\\
%   \cE_{>0} &= \frac{1}{Nq^2} \sum_{\vect{x} \in \{1,\dots,q\}^2} \sum_{m \in \Z}\hspace{2mm}\sum_{\substack{\vect{r} \Mod{q}\\ r_1,r_2\neq 0}} \mathbbm{1}_{\frac{1}{N}I}(\beta(\vect{x}) + m )  e \left(-\frac{\vect{r}\cdot \vect{x}}{q}\right) \left( \prod_{i=1}^m F_N(r_i)\right).\\
% \end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ------------------Prop: bound E-----------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{proposition} \label{prop:bound E}
  In the limit $q \to \infty$ we have:

  \begin{align}
    \cE \to 0 \label{bound E}
  \end{align}
    

\end{proposition}


To prove Proposition \ref{prop:bound E} we will use some Fourier analysis to reduce the problem to estimating and summing stationary phase integrals: First apply the Poisson summation formula to the sum over $m$ (with $f_k(x) := \frac{bk}{q}\sqrt{x}$):


\begin{align*}
  \cE = \frac{1}{Nq^2}\hspace{2mm}\sum_{\substack{\vect{r} \Mod{q}\\ \vect{r}\neq 0}} \left( \prod_{i=1}^m F_N(r_i)\right)  \sum_{\vect{x} \in \{1,\dots,q\}^2} \sum_{k \in \Z} \wh{\mathbbm{1}_{\frac{1}{N}I}}(k)  e\left(-f_k(x_1)-\frac{r_1x_1}{q}\right)  e\left(f_k(x_2)-\frac{r_2x_2}{q}\right) .
\end{align*}
To keep the notation manageable set



\begin{align*}
  \cE^{\vect{r}} = \sum_{\vect{x} \in \{1,\dots,q\}^2} \sum_{k \in \Z} \wh{\mathbbm{1}_{\frac{1}{N}I}}(k)  e\left(-f_k(x_1)-\frac{r_1x_1}{q}\right)  e\left(f_k(x_2)-\frac{r_2x_2}{q}\right) .
\end{align*}
Now since $f_k(x)$ is twice continuously differentiable on $(1,q)$ and $f^\prime$ is monotone, we can apply the 'truncated Poisson summation formula' {\cite[Lemma 5.4.3]{Huxley1996}} to the sum over $x_1$


\begin{align*}
  \begin{aligned}
    \cE^{\vect{r}} &=   \sum_{k \in \Z}\wh{\mathbbm{1}_{\frac{1}{N}I}}(k)\sum_{x_2 \in \{1,\dots,q\}}  e\left(f_k(x_2)-\frac{r_2x_2}{q}\right)  \sum_{\substack{q(A-\frac{1}{4}) \le r \le q(B + \frac{1}{4})\\ r = r_1 \Mod{q}}}   \int_{1}^q   e\left(-f_k(x)-\frac{r x}{q}\right)dx  \\
  & \phantom{++} + \cO\left(\log q\right)   \sum_{k \in \Z_{\neq 0}}\abs{\wh{\mathbbm{1}_{\frac{1}{N}I}}(k)}   \abs{\sum_{x_2 \in \{1,\dots,q\}}e\left(f_k(x_2)-\frac{r_2x_2}{q}\right)}
  \end{aligned}
\end{align*}
where $A := \min_{x \in (1,q)} -f^{\prime}_k(x) = - \frac{bk}{2q}$ and $B := \max_{x \in (1,q)} - f^\prime_k(x) = - \frac{bk}{2q^{1.5}}$.

We can apply this argument again to the sum in $x_2$ to get

\begin{align} \label{Er}
  \begin{aligned}
    \cE^{\vect{r}} &= \cO\left(\log q\right)   \sum_{k \in \Z_{\neq 0}}\abs{\wh{\mathbbm{1}_{\frac{1}{N}I}}(k)}   \abs{\sum_{x_2 \in \{1,\dots,q\}}e\left(f_k(x_2)-\frac{r_2x_2}{q}\right)}\\
    & + \sum_{k \in \Z}\wh{\mathbbm{1}_{\frac{1}{N}I}}(k) \sum_{\substack{q(A-\frac{1}{4}) \le r, r^{\prime} \le q(B + \frac{1}{4})\\ r = r_1 \Mod{q}\\ r^\prime = -r_2 \Mod{q}}}\int_{1}^q \int_1^q   e\left(-f_k(x)-\frac{r x}{q}\right)   e \left(f_k(x') + \frac{r^\prime x^\prime}{q}\right)  dx'dx
  \end{aligned}
\end{align}







\subsection{Stationary Phase Integrals}
\label{ss:Stationary Phase Integrals}



The goal now is to apply a stationary phase integral. However, this is not an immediate consequence of (for example) {\cite[Lemma 5.5.2]{Huxley1996}}, since we do not have sufficient control on the derivatives of $h(x):= -f_k(x) - \frac{rx}{q}$. Moreover the domain of integration grows very quickly and we need very good control of the error term. Therefore we need to adapt the arguments in {\cite[Lemma 5.5.2]{Huxley1996}} to prove:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -----------------------Prop: Stat. Phase--------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{proposition}[Stationary Phase Integral]\label{prop:SPI}
  For $0 \neq r = r_1 \Mod{q}$ and $q(A - \frac{1}{4}) \le r \le q(B+\frac{1}{4})$ and assuming $\gamma \in (1,q)$. As $q \to \infty$ we have:

  \begin{align} \label{Stationary}
    \int_1^qe\left(-f_k(x)-\frac{r x}{q}\right)dx = \frac{e(h(\gamma) + \frac{1}{8})}{\sqrt{h^{\prime \prime}(\gamma)}} + \cO\left(\frac{\gamma^{3/4}}{k^{1/2}}\right).    %\cO\left(\max\left( \frac{1}{h^\prime(q)}, \frac{\gamma^{3/4}}{k^{1/2}}\right)\right) +  \cO\left(\max\left(\frac{e(h(1))}{2\pi i h^\prime(1)}, \frac{\gamma^{3/4}}{k^{1/2}}\right)\right) + \cO\left( \frac{\gamma^{1/2}}{k}  \right) 
  \end{align}
  
\end{proposition}


\begin{proof}

  Fix a small constant $c_1<1$ independent of $q$ and set $u = c_1\gamma$. In that case we have $\abs{h^\prime(u)} = \frac{\eta_1 k}{\gamma^{1/2}}$. 


  First, assume $u>1$ and consider

  \begin{align}
    \begin{aligned}\label{(1,u)}
    \int_{1}^u e(h(x))dx &= \left[\frac{e(h(x))}{2\pi i h^\prime(x)}\right]_{x=1}^u + \frac{1}{2\pi i} \int_{1}^u \frac{h^{\prime\prime}(x)e(h(x))}{h^\prime(x)^2}dx\\
    & = \left[\frac{e(h(x))}{2\pi i h^\prime(x)}\right]_{x=1}^u + \cO\left( \int_{h^\prime(u)}^{h^\prime(1)} \frac{1 }{y^2}dx\right)\\ 
    & = \left[\frac{e(h(x))}{2\pi i h^\prime(x)}\right]_{x=1}^u + \cO\left( \frac{\gamma^{1/2}}{k}\right)\\
    \end{aligned}
  \end{align}
  \color{red} If $u <1$ then do the same thing as we do below for $v$\color{black}

  
  Fix a constant $c_2 >1$, independent of $q$ and all other variables and set $\wt{v}> \gamma$ to be the unique point for which $\abs{h^\prime(\wt{v})} = \frac{k^{1/2}}{\gamma^{3/4}}$. Now we let

  \begin{align*}
    v : =
    \begin{cases}
      c_2\gamma & \mbox{ if } c_2\gamma < q\\
      q         & \mbox{ if } \wt{v} < q \le  c_2\gamma\\
      \wt{v}         & \mbox{ if } \wt{v}\ge q \\
    \end{cases}.
  \end{align*}
  Thus there are three cases, if $v = q$ then:

  \begin{align} \label{v=q}
    \abs{\int_v^q e((h(x))dx} = 0.
  \end{align}
  
  If $v = \wt{v}$

  \begin{align*}
    \abs{\int_v^q e((h(x))dx} \le \abs{\wt{v} - \gamma_r}.
  \end{align*}
  Now note that

  \begin{align*}
    \abs{h^\prime(\wt{v}) - h^\prime(\gamma)} = \frac{k^{1/2}}{\gamma^{3/4}}
  \end{align*}
  Inserting the definition of $h^\prime$ then implies

  \begin{align*}
    \wt{v} = \frac{\gamma}{\left(1 - \frac{q}{bk^{1/2}\gamma^{1/2}}\right)^2}
  \end{align*}
  and hence

  \begin{align} \label{v=v tilde}
    \abs{\int_v^q e((h(x))dx} \le C \frac{\gamma^{3/4}}{k^{1/2}},
  \end{align}
  for some constant $C< \infty$. 






  
  Furthermore, if $v = c_2\gamma$, we can use the first derivative test {\cite[Lemma 5.1.2]{Huxley1996}} to show:
    \begin{align*}
      \int_v^qe(h(x))dx&= \left[\frac{e(h(x))}{2\pi i h^\prime(x)}\right]_{x=v}^q + \frac{1}{2\pi i} \int_{v}^q \frac{h^{\prime\prime}(x)e(h(x))}{h^\prime(x)^2}dx\\
      & = \left[\frac{e(h(x))}{2\pi i h^\prime(x)}\right]_{x=v}^q + \cO\left(\frac{V}{\min \abs{h^\prime(x)}} \right)   \\
    \end{align*}
    where $V$ is the total variation of $h^{\prime\prime}(x)/h^\prime(x)^2$ plus the modulus at $x = v$. Therefore

    \begin{align}
      \begin{aligned}\label{(v,q)}
      \frac{V}{\min\abs{h^\prime(x)}} &= \frac{\gamma^{1/2}}{k}  \int_v^q \abs{\frac{h^{(3)}(x)}{h^\prime(x)^2} - \frac{2h^{\prime\prime}(x)^2}{h^{\prime}(x)^3}}dx + \frac{\gamma^{1/2}}{k} \frac{h^{\prime\prime}(v)}{h^{\prime}(v)^2}\\
                                      & = \cO\left( \frac{\gamma^{1/2}}{k}  \int_v^q \abs{\frac{ kb \gamma}{k^2q x^{5/2}}} + \abs{\frac{\gamma^{3/2} k^2b^2}{k^3 q^2 x^3}}dx + \frac{\gamma^{1/2}}{k} \frac{kb \gamma}{qk^2 \gamma^{3/2}} \right)\\
                                      & = \cO\left( \frac{\gamma^{1/2}}{k} \int_v^q \abs{\frac{  \gamma}{k x^{5/2}}} + \abs{\frac{\gamma^{3/2} }{k  x^3}}dx  + \frac{1}{k^2} \right)\\
                                      & = \cO\left( \frac{\gamma^{1/2}}{k}  \frac{  \gamma}{k \gamma^{3/2}} + \frac{\gamma^{3/2} }{k  \gamma^2}  + \frac{1}{k^2} \right) = \cO\left(\frac{1}{k^2}\right)\\
      \end{aligned}
    \end{align}

    Now working in $[u,v]$, set $T = \frac{kb \gamma^{1/2}}{q}$ and $M= \gamma$. Then for $j=2,3,4$, there exist constants $0< C_j < \infty$ such that

  \begin{align*}
    \abs{h^{(j)}(x)} \le C_j\frac{T}{M^j} \qquad , \qquad h^{\prime\prime}(x)\ge h^{\prime\prime}(v) \ge C_2^{-1}  \frac{T}{M^2}
  \end{align*}
  Thus we can apply {\cite[Lemma 5.5.2]{Huxley1996}} to say:

  \begin{align}
    \begin{aligned}\label{(u,v)}
    \int_u^vh(x) dx &= \frac{e(h(\gamma)+1/8)}{\sqrt{h^{\prime\prime}(\gamma)}} + \frac{e(h(v))}{2\pi i h^{\prime}(v)} - \frac{e(h(u))}{2\pi i h^{\prime}(u)}
                      + \cO\left(\frac{M}{T^{3/2}} + \frac{M^4}{T^2}\left(\frac{h^{\prime \prime}(\gamma)}{k \eta}  \right)^3  \right)\\
     &= \frac{e(h(\gamma)+1/8)}{\sqrt{h^{\prime\prime}(\gamma)}} + \frac{e(h(v))}{2\pi i h^{\prime}(v)} - \frac{e(h(u))}{2\pi i h^{\prime}(u)}
       + \cO\left(\frac{\gamma}{k^{3/2}\gamma^{3/4}} + \frac{\gamma^3}{k^2}\left(\frac{h^{\prime \prime}(\gamma)}{k \eta}  \right)^3  \right)\\
     &= \frac{e(h(\gamma)+1/8)}{\sqrt{h^{\prime\prime}(\gamma)}} + \frac{e(h(v))}{2\pi i h^{\prime}(v)} - \frac{e(h(u))}{2\pi i h^{\prime}(u)}
     + \cO\left(\frac{\gamma^{1/4}}{k^{3/2}} + \frac{1}{k^2\gamma^{3/2}} \right).
     \end{aligned}
  \end{align}
  Therefore, putting \eqref{(1,u)}, \eqref{(v,q)} and \eqref{(u,v)} together (and using that $\gamma >1$) imply \eqref{Stationary}.




  


\end{proof}



This same argument can be used to prove:



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -----------------------Prop: Large gamma -------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{proposition}[Large $\gamma$ bound]\label{prop:gamma large}
  For $r = r_1 \Mod{q}$ and $q(A - \frac{1}{4}) \le r \le q(B+\frac{1}{4})$ and assuming $\gamma > q$. As $q \to \infty$ we have:

  \textbf{If $q < \gamma < 1.1q$:}
  
  \begin{align} \label{gamma not huge}
    \int_1^qe\left(-f_k(x)-\frac{r x}{q}\right)dx = \cO\left( \frac{\gamma^{3/4}}{k^{1/2}}\right)
  \end{align}

  \textbf{If $\gamma > 1.1 q$:}
  
  \begin{align} \label{gamma huge}
    \int_1^qe\left(-f_k(x)-\frac{r x}{q}\right)dx = \cO\left( \frac{q^{1/2}}{k}\right)
  \end{align}
  
  
\end{proposition}


\subsection{Proof of Proposition \ref{prop:bound E}}


Now, if we assume that $r_1,r_2 \neq 0$, these stationary phase integrals are enough to bound $\cE^{\vect{r}}$ Note first that using Proposition \ref{prop:SPI} and Proposition \ref{prop:gamma large}

\begin{align*}
  \sum_{\substack{q(A-\frac{1}{4})\le r \le q(B+\frac{1}{4})\\ r = r_1\Mod{q}}}\int_1^q e(h(x))dx \le  \sum_{\substack{q(A-\frac{1}{4})\le r \le q(B+\frac{1}{4})\\ r = r_1\Mod{q}}} \left(\frac{\gamma^{3/4}}{k^{1/2}} \mathbbm{1}(\gamma < 1.1 q) + \frac{q^{1/2}}{k} \mathbbm{1}(\gamma > 1.1 q)\right).
\end{align*}
Now note that $\gamma = \frac{kb}{2r}$, thus $\gamma > 1.1 q$ is only possible for at most one single $r$ (given that $r_1$ is fixed and $k < q$) hence


\begin{align*}
  \sum_{\substack{q(A-\frac{1}{4})\le r \le q(B+\frac{1}{4})\\ r = r_1\Mod{q}}}\int_1^q e(h(x))dx \le \frac{q^{1/2}}{k} + \frac{1}{k^{1/2}}  \sum_{\substack{q(A-\frac{1}{4})\le r \le q(B+\frac{1}{4})\\ r = r_1\Mod{q}}} \left(\frac{kb}{2r}\right)^{3/2} \mathbbm{1}(\gamma < 1.1 q) .
\end{align*}
Finally since the sum of $\frac{1}{r^{3/2}}$ is dominated by the largest term  in the sum, we conclude

\begin{align*}
  \sum_{\substack{q(A-\frac{1}{4})\le r \le q(B+\frac{1}{4})\\ r = r_1\Mod{q}}}\int_1^q e(h(x))dx = \cO\left( \frac{q^{1/2}}{k} + \frac{q^{3/4}}{k^{1/2}}\right) .
\end{align*}

Now if we return to \eqref{Er} and apply the same argument to the sum over $r^\prime$ we get that

\begin{align} \label{Er bound >0}
  \cE^{\vect{r}} = \cO \left( \frac{1}{N} \sum_{\substack{k \in \Z \\ \abs{k < q}}} \frac{q^{3/2}}{k} \right) = \cO \left(\frac{q^{3/2}\log q}{N}\right)
\end{align}

Now suppose $r_1 =0$. Then we can use \eqref{Er} to write (ignoring the logarithmic error term which can be easily controlled using the stationary phase integrals.

\begin{align*}
    \cE^{\vect{r}} &\sim  \sum_{k \in \Z}\wh{\mathbbm{1}_{\frac{1}{N}I}}(k) \sum_{\substack{q(A-\frac{1}{4}) \le r, r^{\prime} \le q(B + \frac{1}{4})\\ r = 0 \Mod{q}\\ r^\prime = -r_2 \Mod{q}}}\int_{1}^q \int_1^q   e\left(-f_k(x)-\frac{r x}{q}\right)   e \left(f_k(x') + \frac{r^\prime x^\prime}{q}\right)  dx'dx.
\end{align*}
Now we separate the term $r =0$ and use the above argument to bound what remains:


\begin{align*}
    \cE^{\vect{r}} &= \cO\left(\frac{q^{3/2}\log q }{N}\right) +   \sum_{k \in \Z}\wh{\mathbbm{1}_{\frac{1}{N}I}}(k) \sum_{\substack{q(A-\frac{1}{4}) \le  r^{\prime} \le q(B + \frac{1}{4})\\ r^\prime = -r_2 \Mod{q}}}\int_{1}^q \int_1^q   e\left(-f_k(x)\right)   e \left(f_k(x') + \frac{r^\prime x^\prime}{q}\right)  dx'dx.
\end{align*}
Now using the first derivative test we have the following bound:

\begin{align*}
  \abs{\int_1^q e(-f_k (x)) dx} &\le \abs{\left[ \frac{1}{2\pi i f_k^\prime(y)}\right]_{y=1}^q} + \int_1^q \frac{f_k^{\prime\prime}(x)}{f_k^\prime(x)^2} dx\\
                                & = \cO\left(\frac{q^{1/2}}{k} \right) + \int_1^q \frac{q}{kb x^{1/2}}dx\\
                                & =  \cO\left(\frac{q^{1/2}}{k} \right).
\end{align*}
Putting this bound together with the above stationary phase integrals gives:

\begin{align} \label{Er bound 0} 
  \begin{aligned}
    \cE^{\vect{r}} &= \cO\left(\frac{q^{3/2}\log q }{N}\;\;  +\;\; \frac{1}{N} \sum_{k \in \Z} \frac{q^{1/2}}{k} \sum_{\substack{q(A-\frac{1}{4}) \le  r^{\prime} \le q(B + \frac{1}{4})\\ r^\prime = -r_2 \Mod{q}}} \frac{\gamma_{r^\prime}^{3/4}}{k^{1/2}}\right)\\
     &= \cO\left(\frac{q^{3/2}\log q }{N}\;\;  +\;\; \frac{1}{N} \sum_{k \in \Z}  \frac{q^{5/4}}{k^{3/2}}\right)        = \cO\left(\frac{q^{3/2}\log q }{N}\right)\\  
\\  
  \end{aligned}
\end{align}
Inserting \eqref{Er bound >0} and \eqref{Er bound 0} into the definition of $\cE$ and applying the bound \eqref{F bound} imply

\begin{align*}
  \cE \le \frac{\log(q)^3 q^{3/2}}{N^2}  \to 0
\end{align*}
(where we use that $N > q^{3/4 + \delta}$). This concludes the proof of \eqref{bound E}. 

\qed

